Solving Linear Inverse Problems Using GAN Priors: An Algorithm with Provable Guarantees

In recent works, both sparsity-based methods as well as learning-based methods have proven to be successful in solving several challenging linear inverse problems. However, sparsity priors for natural signals and images suffer from poor discriminative capability, while learning-based methods seldom provide concrete theoretical guarantees. In this work, we advocate the idea of replacing hand-crafted priors, such as sparsity, with a Generative Adversarial Network (GAN) to solve linear inverse problems such as compressive sensing. In particular, we propose a projected gradient descent (PGD) algorithm for effective use of GAN priors for linear inverse problems, and also provide theoretical guarantees on the rate of convergence of this algorithm. Moreover, we show empirically that our algorithm demonstrates superior performance over an existing method of leveraging GANs for compressive sensing.

==> common/conclusion.tex <==
\section{Conclusion}


==> common/fig_curve.tex <==
\begin{figure*}
	\begin{subfigure}[t]{0.48\textwidth}
		\includegraphics[width=\textwidth]{..\fig\mnist_curve.png}
		\caption{We show original images (top row) and reconstructions by Lasso (middle row) and our algorithm (bottom row).}
		\label{fig:mnist-reconstr}
	\end{subfigure}\hfill%
	\begin{subfigure}[t]{0.48\textwidth}
		\includegraphics[width=\textwidth]{mnist_superres_orig_blurred_lasso_vae-gen.pdf}
		\caption{We show original images (top row), low resolution version of original images (middle row) and reconstructions (last row).}
		\label{fig:mnist-superres}
	\end{subfigure}
	\caption{Results on MNIST\@. Reconstruction with 100 measurements (left) and Super-resolution (right)}
\end{figure*}

